Space-time block preconditioning for incompressible flow

Parallel-in-time methods have become increasingly popular in the simulation of time-dependent numerical PDEs, allowing for the efficient use of additional MPI processes when spatial parallelism saturates. Most methods treat the solution and parallelism in space and time separately. In contrast, all-at-once methods solve the full space-time system directly, largely treating time as simply another spatial dimension. All-at-once methods offer a number of benefits over separate treatment of space and time, most notably significantly increased parallelism and faster time-to-solution (when applicable). However, the development of fast, scalable all-at-once methods has largely been limited to time-dependent (advection-)diffusion problems. This paper introduces the concept of space-time block preconditioning for the all-at-once solution of incompressible flow. By extending well-known concepts of spatial block preconditioning to the space-time setting, we develop a block preconditioner whose application requires the solution of a space-time (advection-)diffusion equation in the velocity block, coupled with a pressure Schur complement approximation consisting of independent spatial solves at each time-step, and a space-time matrix-vector multiplication. The new method is tested on four classical models in incompressible flow. Results indicate perfect scalability in refinement of spatial and temporal mesh spacing, perfect scalability in nonlinear Picard iterations count when applied to a nonlinear Navier-Stokes problem, and minimal overhead in terms of number of preconditioner applications compared with sequential time-stepping.

==> sec/eigs.tex <==
\begin{section}{Eigenvalues analysis}
\label{sec::eigs}
In this section, we analyse the clustering properties of the preconditioners
introduced in \cref{sec::precon}. Since we intend to use GMRES as an iterative
solver for \cref{eqn::STdisc}, simply studying the eigenvalue distribution of
the preconditioned system is not sufficient to guarantee quick convergence
\cite{convGMRES}, especially since the target system is highly non-symmetric;
nonetheless, poor clustering is usually associated with slow convergence, so at
the least this analysis can give us some insight on when the preconditioner
might behave poorly. In this section we only consider Stokes equations (or
equivalently, we pick $\bb{w}\equiv0$ in \cref{eqn::Oseen}). This has the effect
of greatly simplifying the analysis, since most of the operators involved become
self-adjoint.

Our analysis is similar to the one conducted in \cite{andyFIT}: the aim is to
provide bounds on the solutions to the generalised eigenvalue problems
\begin{equation}
  \left[\begin{array}{cc}
    F_{\bb{u}} & B^T \\
    B          &
  \end{array}\right]\left[\begin{array}{c}
    \bb{u} \\
    \bb{p} 
  \end{array}\right]=\lambda\left[\begin{array}{cc}
    F_{\bb{u}} &  \\
               & -X
  \end{array}\right]\left[\begin{array}{c}
    \bb{u} \\
    \bb{p}
  \end{array}\right],
  \label{eqn::GEPbDprec}
\end{equation}
in the case of the block diagonal preconditioner \cref{eqn::PD}, or
\begin{equation}
  \left[\begin{array}{cc}
    F_{\bb{u}} & B^T \\
    B          &
  \end{array}\right]\left[\begin{array}{c}
    \bb{u} \\
    \bb{p} 
  \end{array}\right]=\lambda\left[\begin{array}{cc}
    F_{\bb{u}} & B^T\\
               & -X
  \end{array}\right]\left[\begin{array}{c}
    \bb{u} \\
    \bb{p}
  \end{array}\right],
  \label{eqn::GEPbTprec}
\end{equation}
for the block triangular version \cref{eqn::PT}. Both systems present
$\lambda=1$ as a solution with multiplicity $N_\bb{u}$; the remaining ones are
given either by satisfying
\begin{equation}
  \left(\frac{BF_{\bb{u}}^{-1}B^T}{\lambda-1} + \lambda X\right)\bb{p} = 0\quad\Longleftrightarrow \\
  \left(X^{-1}BF_{\bb{u}}^{-1}B^T -\lambda(  1-\lambda)I\right)\bb{p} = 0,\\
\end{equation}
for the block diagonal preconditioner, or
\begin{equation}
  \left(X^{-1}BF_{\bb{u}}^{-1}B^T - \lambda I\right)\bb{p} = 0,\\
\end{equation}
for the block triangular one. In either case, the general eigenvalues of
\cref{eqn::GEPbDprec} or \cref{eqn::GEPbTprec} directly relate to the
eigenvalues of the matrix $X^{-1}BF_{\bb{u}}^{-1}B^T$. Substituting our
approximation to the space-time pressure Schur complement \cref{eqn::XXdef}, we
have that the operator of interest becomes
\begin{equation}
  X^{-1}BF_{\bb{u}}^{-1}B^T \approx M_p^{-1}F_p A_p^{-1}BF_{\bb{u}}^{-1}B^T.
  \label{eqn::GEprob}
\end{equation}
This matrix is block lower triangular, since $F_p$ and $F_{\bb{u}}^{-1}$ both
are and the remaining factors are block diagonal matrices. To find its
eigenvalues, we just need to recover the eigenvalues of the blocks on the main
diagonal. These blocks are all equal to each other (since \cref{eqn::GEprob} is
also block Toeplitz), and consist of the operator
\begin{equation}
  \mc{M}_p^{-1}\mc{F}_p\mc{A}_p^{-1}\mc{B}\mc{F}_{\bb{u}}^{-1}\mc{B}^T.
  % = \mc{B}\left(\frac{\mc{M}_{\bb{u}}}{\Delta t}+\mu\mc{A}_{\bb{u}}\right)^{-1}\mc{B}^T\left(\frac{\mc{A}_p^{-1}}{\Delta t}+\mu\mc{M}_p^{-1}\right),
  \label{eqn::blockGEP}
\end{equation}
% \paragraph{Stokes}
% In the case of the time-dependent Stokes equation, the block \cref{eqn::blockGEP} reduces to
% \begin{equation}
%   \mc{M}_p^{-1}\hat{\mc{F}}_p\mc{A}_p^{-1}\mc{B}\hat{\mc{F}}_{\bb{u}}^{-1}\mc{B}^T
%   = \left(\frac{\mc{A}_p^{-1}}{\Delta t}+\mu\mc{M}_p^{-1}\right)\mc{B}\left(\frac{\mc{M}_{\bb{u}}}{\Delta t}+\mu\mc{A}_{\bb{u}}\right)^{-1}\mc{B}^T,
%   \label{eqn::blockGEPstokes}
% \end{equation}
% The factors containing mass and stiffness matrix are both symmetric positive definite, and can be decomposed into a product of their matrix square roots. Rearranging the matrix products, we have that the matrix above is similar to
% \begin{equation}
%   \cref{eqn::blockGEPstokes} \sim \left(\frac{\mc{A}_{p}^{-1}}{\Delta t}+\mu\mc{M}_{p}^{-1}\right)^{\frac{1}{2}}\mc{B}\left(\frac{\mc{M}_{\bb{u}}}{\Delta t}+\mu\mc{A}_{\bb{u}}\right)^{-1}\mc{B}^T\left(\frac{\mc{A}_{p}^{-1}}{\Delta t}+\mu\mc{M}_{p}^{-1}\right)^{\frac{1}{2}}.
%   \label{eqn::blockGEPstokes2}
% \end{equation}
% We recover bounds on the eigenvalues of this matrix by analysing its field of values, which is given by
% \begin{equation}
% \begin{split}
%   & \frac{\left\langle\left(\frac{\mc{A}_{p}^{-1}}{\Delta t}+\mu\mc{M}_{p}^{-1}\right)^{\frac{1}{2}}\mc{B}\left(\frac{\mc{M}_{\bb{u}}}{\Delta t}+\mu\mc{A}_{\bb{u}}\right)^{-1}\mc{B}^T\left(\frac{\mc{A}_{p}^{-1}}{\Delta t}+\mu\mc{M}_{p}^{-1}\right)^{\frac{1}{2}}p,p\right\rangle}{\left\langle p,p\right\rangle}\\
%   =&\frac{\left\langle\left(\mc{M}_{\bb{u}}+\tau\mc{A}_{\bb{u}}\right)^{-1}z,z\right\rangle}{\left\langle z,z\right\rangle}\frac{\left\langle \mc{B}\mc{B}^Ty,y\right\rangle}{\left\langle y,y\right\rangle}\frac{\left\langle\left(\mc{A}_p^{-1}+\tau\mc{M}_p^{-1}\right)p,p\right\rangle}{\left\langle p,p\right\rangle}\\
%   =&\frac{\left\langle\mc{B}\left(\mc{M}_{\bb{u}}+\tau\mc{A}_{\bb{u}}\right)^{-1}\mc{B}^Ty,y\right\rangle}{\left\langle y,y\right\rangle}\frac{\left\langle\left(\mc{A}_p^{-1}+\tau\mc{M}_p^{-1}\right)p,p\right\rangle}{\left\langle p,p\right\rangle},
% \end{split}
% \label{eqn::blockGEPstokesFOV}
% \end{equation}
% where $\tau=\mu\Delta t$, $z=\mc{B}^Ty$, $y=\left(\frac{\mc{A}_p^{-1}}{\Delta t}-\mu\mc{M}_p^{-1}\right)^{\frac{1}{2}}p$, while $p$ can vary freely. We can then bound the field of values of \cref{eqn::blockGEPstokes2} using independently the field of values of the matrices appearing in \cref{eqn::blockGEPstokesFOV}.
% Since all the matrices involved are SPD \textcolor{red}{- what about $\mc{B}\mc{B}^T$? Is it definite?} (they are all sums and/or inverses of SPD), their field of values reduces to the interval between their minimum and maximum eigenvalues. Moreover, for a \textcolor{red}{quasi-uniform} discretisation defined on a regular 2D domain, with discretisation parameter $h$, we have:
% \begin{equation}
% \begin{array}{lcccll}
%   c_\mc{M}^{\bb{u}} h^2 & \leq & \lambda(\mc{M}_{\bb{u}})        & \leq & C_\mc{M}^{\bb{u}} h^2 &\quad\quad\text{\cite[Prop.1.30]{andyFIT}}\\
%   c_\mc{A}^{\bb{u}} h^2 & \leq & \lambda(\mc{A}_{\bb{u}})        & \leq & C_\mc{A}^{\bb{u}}     &\quad\quad\text{\cite[Thm.1.33]{andyFIT} }\\
%   % c_\mc{B}       h^2 & \leq & \lambda(\mc{B}\mc{B}^T) & \leq & C_\mc{B}           &\quad\quad\textcolor{red}{\text{Well, this must be proven...}}\\
%   \label{eqn::massStiffBound}
% \end{array},
% \end{equation}
% \textcolor{red}{and similarly for mass and stiffness matrix defined on the pressure field.}
To be more precise, we should write $\tilde{\mc{A}}_p$ rather than $\mc{A}_p$;
however, we drop the tilde in light of the considerations from
\cref{sec::precon::Apdef}. This is also helpful in simplifying the upcoming
analysis. We separate the factors in \cref{eqn::blockGEP} as
\begin{equation}
  \left(\mc{A}_p\mc{F}_p^{-1}\mc{M}_p\right)^{-1}\qquad\text{and}\qquad\mc{B}\mc{F}_{\bb{u}}^{-1}\mc{B}^T,
  % = \mc{B}\left(\frac{\mc{M}_{\bb{u}}}{\Delta t}+\mu\mc{A}_{\bb{u}}\right)^{-1}\mc{B}^T\left(\frac{\mc{A}_p^{-1}}{\Delta t}+\mu\mc{M}_p^{-1}\right),
  \label{eqn::blockGEPfact}
\end{equation}
and notice that, under the simplifications introduced in
\cref{sec::precon::Apdef}, the operator on the left is also \emph{Symmetric
Positive Definite} (SPD), since
\begin{equation}
  \mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p} = \left(\frac{\mc{A}_{p}^{-1}}{\Delta t}+\mu\mc{M}_{p}^{-1}\right)^{-1},
  \label{eqn::XisSPD}
\end{equation}
where both $\mc{A}_p$ and $\mc{M}_p$ are SPD. The operator \cref{eqn::blockGEP}
becomes then reminiscent of another preconditioned system, which involves a
single block in the monolithic space-time matrix: showing that the eigenvalues
of \cref{eqn::blockGEP} are clustered reduces to proving the spectral
equivalence between the two matrices in \cref{eqn::blockGEPfact}. This in turn
can be investigated by considering the following \emph{generalised singular
value problem}\footnote{This procedure is akin to the analysis performed in
\cite[Chap.~3.5]{andyFIT} for the Stokes equations. In that case, the aim was to
prove the spectral equivalence between the chosen preconditioner $\mc{M}_{p}$
and the pressure Schur complement $\mc{B}\mc{A}_{\bb{u}}^{-1}\mc{B}^{T}$: the
generalised singular value problem considered for this purpose was
\begin{equation}
\left[\begin{array}{cc}
         & \mc{B}^T\\
  \mc{B} &  
\end{array}\right] \left[\begin{array}{c}
  \bb{u}\\
  \bb{p}
\end{array}\right] = \sigma\left[\begin{array}{cc}
  \mc{A}_{\bb{u}} &                \\
                  & \mc{M}_p
\end{array}\right] \left[\begin{array}{c}
  \bb{u} \\
  \bb{p}
\end{array}\right].
\end{equation}
In our case the structure is identical, but we are proposing to approximate the
space-time pressure Schur complement $\mc{B}\mc{F}_{\bb{u}}\mc{B}^T$ using
$\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}$ instead.}
\begin{equation}
\left[\begin{array}{cc}
         & \mc{B}^T\\
  \mc{B} &  
\end{array}\right] \left[\begin{array}{c}
  \bb{u}\\
  \bb{p}
\end{array}\right] = \sigma\left[\begin{array}{cc}
  \mc{F}_{\bb{u}} &\\
                  & \mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}
\end{array}\right] \left[\begin{array}{c}
  \bb{u}\\
  \bb{p}
\end{array}\right].
\end{equation}
In fact, we have that the following relationship holds between the generalised
singular values and the Rayleigh quotient of the matrices in
\cref{eqn::blockGEPfact}:
\begin{equation}
  \frac{\left\langle\mc{B}\mc{F}_{\bb{u}}^{-1}\mc{B}^{T}\bb{q},\bb{q}\right\rangle}{\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\bb{q},\bb{q}\right\rangle}
  = \sigma^2
  =\frac{\left\langle\mc{B}^T\mc{M}_{p}^{-1}\mc{F}_{p}\mc{A}_{p}^{-1}\mc{B}\bb{v},\bb{v}\right\rangle}{\left\langle \mc{F}_{\bb{u}} \bb{v},\bb{v}\right\rangle},
  % \quad\text{or}\quad\frac{\left\langle\mc{B}\mc{F}_{\bb{u}}^{-1}\mc{B}^{T}q,q\right\rangle}{\left\langle\mc{B}\mc{M}_{p}^{-1}\mc{B}^T\mc{F}_{p}^{-1}\mc{M}_{p}q,q\right\rangle}
  \label{eqn::specBounds0}
\end{equation}
for all $(\bb{v},\bb{q})\in V_h(\Omega)\times Q_h(\Omega)$ such that
$\left\langle\mc{F}_{\bb{u}}\bb{v},\bb{v}\right\rangle=\left\langle\mc{A}_p\mc{F}_p^{-1}\mc{M}_p\bb{q},\bb{q}\right\rangle$.
Proving their spectral equivalence reduces then to bounding $\sigma^2$,
\emph{i.e.}, finding two scalars $\ubar{\sigma}^2$ and $\bar{\sigma}^2$ such
that
\begin{equation}
  \ubar{\sigma}^2\leq\frac{\left\langle\mc{B}\mc{F}_{\bb{u}}^{-1}\mc{B}^{T}\bb{q},\bb{q}\right\rangle}{\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\bb{q},\bb{q}\right\rangle}
    = \sigma^2
    =\frac{\left\langle\mc{B}^T\mc{M}_{p}^{-1}\mc{F}_{p}\mc{A}_{p}^{-1}\mc{B}\bb{v},\bb{v}\right\rangle}{\left\langle \mc{F}_{\bb{u}} \bb{v},\bb{v}\right\rangle}
       % \quad\text{or}\quad\frac{\left\langle\mc{B}\mc{F}_{\bb{u}}^{-1}\mc{B}^{T}q,q\right\rangle}{\left\langle\mc{B}\mc{M}_{p}^{-1}\mc{B}^T\mc{F}_{p}^{-1}\mc{M}_{p}q,q\right\rangle}
  \leq\bar{\sigma}^2,
  \label{eqn::specBounds}
\end{equation}
either $\forall \bb{q}\in Q_h(\Omega)$ or $\forall \bb{v}\in V_h(\Omega)$. To
simplify notation in the following derivation, we introduce these norms for our
the discrete pressure space:
\begin{equation}
\begin{split}
  \|\bb{q}\|_{p}^2 = \left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\bb{q},\bb{q}\right\rangle\qquad\text{and}\qquad
  \|\bb{q}\|_{0}^2 = \left\langle\mc{M}_{p}\bb{q},\bb{q}\right\rangle.
\end{split}
\label{eqn::normsP}
\end{equation}
Notice $\|\bb{q}\|_0$ is simply the $L^2$-norm. For the discrete velocity space, instead, we define
\begin{equation}
  \|\bb{v}\|_{\bb{u}}^2 = \left\langle\mc{F}_{\bb{u}}\bb{v},\bb{v}\right\rangle\qquad\text{and}\qquad
  \|\bb{v}\|_{1}^2      = \left\langle\mc{A}_{\bb{u}}\bb{v},\bb{v}\right\rangle,
\label{eqn::normsV}
\end{equation}
where $\|\bb{v}\|_1\equiv\|\nabla\bb{v}(\bb{x})\|_0$, the $H_1$-semi-norm.



\paragraph{Upper bound}
We first find $\bar{\sigma}^2$: starting from the Rayleigh quotient on the left of \cref{eqn::specBounds}, we obtain
\begin{equation}
  \frac{\left\langle\mc{B}\mc{F}_{\bb{u}}^{-1}\mc{B}^{T}\bb{q},\bb{q}\right\rangle^{\frac{1}{2}}}{\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\bb{q},\bb{q}\right\rangle^{\frac{1}{2}}}
  =\frac{\left\langle\mc{F}_{\bb{u}}^{-\frac{1}{2}}\mc{B}^{T}\bb{q},\mc{F}_{\bb{u}}^{-\frac{1}{2}}\mc{B}^{T}\bb{q}\right\rangle^{\frac{1}{2}}}{\|\bb{q}\|_p}
  % =\frac{\left\langle\mc{F}_{\bb{u}}^{-\frac{1}{2}}\mc{B}^{T}\bb{q},\bb{w}\right\rangle}{\|\bb{q}\|_p\|\bb{w}\|_0}
  =\frac{|\left\langle\bb{q},\mc{B}\bb{v}\right\rangle|} {\|\bb{q}\|_p\|\bb{v}\|_\bb{u}},
  \label{eqn::simplerRayleighQuotient}
\end{equation}
where we substituted $\bb{v}=\mc{F}_{\bb{u}}^{-1}\mc{B}^{T}\bb{q}$. We focus then on the right-most term, and notice its numerator equals $|\left\langle q(\bb{x}),\nabla\cdot\bb{v}(\bb{x})\right\rangle|$, where $q(\bb{x})$ and $\bb{v}(\bb{x})$ are the functions corresponding to the vectors $\bb{q}$ and $\bb{v}$, according to \cref{eqn::FEvec2fun}. Using Cauchy-Schwarz,
\begin{equation}
  |\left\langle q(\bb{x}),\nabla\cdot\bb{v}(\bb{x})\right\rangle| \leq \|q(\bb{x})\|_0 \|\nabla\cdot\bb{v}(\bb{x})\|_0,
\end{equation}
and moreover, we have
\begin{equation}
  \|\nabla\cdot\bb{v}(\bb{x})\|_0^2 \leq \|\nabla\cdot\bb{v}(\bb{x})\|_0^2 + \|\nabla\times\bb{v}(\bb{x})\|_0^2 = \|\nabla\bb{v}(\bb{x})\|^2_0 =  \|\bb{v}\|^2_1,
\end{equation}
which allows us to write 
\begin{equation}
  \frac{|\left\langle\bb{q},\mc{B}\bb{v}\right\rangle|} {\|\bb{q}\|_p\|\bb{v}\|_\bb{u}}
  \leq \max_{\bb{q}\in Q_h(\Omega)}\frac{\|\bb{q}\|_0}{\|\bb{q}\|_p} \max_{\bb{v}\in V_h(\Omega)}\frac{\|\bb{v}\|_1}{\|\bb{v}\|_\bb{u}},
\end{equation}
at which point finding the upper bound for \cref{eqn::specBounds} becomes an exercise in proving equivalence of norms. For the velocity field, we have:
\begin{equation}
  \|\bb{v}\|_1^2 = \left\langle\mc{A}_{\bb{v}}\bb{v},\bb{v}\right\rangle
  \leq\max\left\{1,\mu^{-1}\right\}\left\langle\left(\frac{\mc{M}_{\bb{u}}}{\Delta t}+\mu\mc{A}_{\bb{u}}\right)\bb{v},\bb{v}\right\rangle
  =   \max\left\{1,\mu^{-1}\right\}\|\bb{v}\|_{\bb{u}}^2.
  \label{eqn::rightBoundV}
\end{equation}
For the pressure field, the analysis requires more care. Firstly, we can write
\begin{equation}
  \frac{\|\bb{q}\|_0^2}{\|\bb{q}\|_p^2}
  =   \frac{\left\langle\mc{M}_{p}q,q\right\rangle}{\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}q,q\right\rangle}
  \leq\frac{\bar{\lambda}(\mc{M}_{p})}{\ubar{\lambda}\left(\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\right)}
  =\bar{\lambda}(\mc{M}_{p})\bar{\lambda}\left(\mc{A}_{p}^{-1}\mc{F}_{p}\mc{M}_{p}^{-1}\right),
  % \leq\frac{\max_{\bb{q}\in Q_h(\Omega)}|W(\mc{M}_{p})|}{\min_{\bb{q}\in Q_h(\Omega)}|W\left(\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\right)|},
  % = \frac{\left\langle\mc{M}_{p}q,q\right\rangle}{\left\langle\mc{\tilde{F}}_{p}^{-1}q,q\right\rangle}
  % = \frac{W(\mc{M}_{p})}{W\left(\left(\frac{\mc{A}_{p}^{-1}}{\Delta t}+\mu\mc{M}_{p}^{-1}\right)^{-1}\right)},
  % = \frac{\left\langle\left(\mc{M}_{p}+\tau\mc{A}_{p}\right)q,q\right\rangle}{\left\langle\mc{A}_{p}q,q\right\rangle}
  %   = \left(\frac{\left\langle\mc{M}_{p}q,q\right\rangle}{\Delta t\left\langle q,q\right\rangle}+\mu\frac{\left\langle\mc{A}_{p}q,q\right\rangle}{\left\langle q,q\right\rangle}\right)\left(\frac{\left\langle\mc{A}_{p}q,q\right\rangle}{\left\langle q,q\right\rangle}\right)^{-1}\\
  % & \leq \frac{1}{\Delta t}\frac{\lambda^{max}(\mc{M}_p)}{\lambda^{min}(\mc{A}_p)} + \mu \frac{\lambda^{max}(\mc{A}_p)}{\lambda^{min}(\mc{A}_p)}
  % \leq \frac{C^p_\mc{M}}{c^p_\mc{A}} + \tau \\
  % \Longrightarrow & \|q\|_0^2 \leq  \left(\frac{C^p_\mc{M}}{c^p_\mc{A}} + \tau \right)\|q\|_p^2,
  \label{eqn::rightBoundPtemp}
\end{equation}
where $\ubar{\lambda}(*)$ and $\bar{\lambda}(*)$ respectively denote the smallest and largest eigenvalues of matrix $(*)$, and we once again exploit the fact that the matrices involved are SPD.
We also notice that
\begin{equation}
  \lambda\left(\mc{A}_{p}^{-1}\mc{F}_{p}\mc{M}_{p}^{-1}\right)= \lambda\left(\frac{\mc{A}_{p}^{-1}}{\Delta t}+\mu\mc{M}_{p}^{-1}\right)\subseteq\left[\frac{\Delta t^{-1}}{\bar\lambda(\mc{A}_p)} + \frac{\mu}{\bar\lambda(\mc{M}_p)}, \frac{\Delta t^{-1}}{\ubar\lambda(\mc{A}_p)} + \frac{\mu}{\ubar\lambda(\mc{M}_p)}\right].
\label{eqn::FOVp2}
\end{equation}
The final ingredient we need to recover an expression for $\bar{\sigma}^2$, is a bound on the eigenvalues of the Galerkin mass and stiffness matrices: for $\Omega\in\mathbb{R}^2$, these are given by
\begin{equation}
\begin{array}{lcccll}
  \ubar{c}_\mc{M}^{(*)} \Delta x^2 & \leq & \lambda(\mc{M}_{(*)}) & \leq & \bar{c}_\mc{M}^{(*)} \Delta x^2 &\quad\quad\text{\cite[Prop.1.30]{andyFIT}},\\[4pt]
  \ubar{c}_\mc{A}^{(*)} \Delta x^2 & \leq & \lambda(\mc{A}_{(*)}) & \leq & \bar{c}_\mc{A}^{(*)}            &\quad\quad\text{\cite[Thm.1.33]{andyFIT} },
  % c_\mc{B}       h^2 & \leq & \lambda(\mc{B}\mc{B}^T) & \leq & C_\mc{B}           &\quad\quad\textcolor{red}{\text{Well, this must be proven...}}\\
  \label{eqn::massStiffBound}
\end{array}
\end{equation}
where $\ubar{c}_\mc{M}$, $\bar{c}_\mc{M}$, $\ubar{c}_\mc{A}$, and $\bar{c}_\mc{A}$ are some constants depending on the \tcr{domain and the }type of discretisation; these bounds hold both for pressure and velocity, $(*)=p$ or $(*)=\bb{u}$, and are valid for a quasi-uniform discretisation defined on a regular 2D domain, with characteristic mesh size $\Delta x$.
Substituting \cref{eqn::massStiffBound} for the pressure variable in \cref{eqn::rightBoundPtemp} gives the upper bound for the equivalence of the norms introduced in \cref{eqn::normsP}:
\begin{equation}
  \frac{\|\bb{q}\|_0^2}{\|\bb{q}\|_p^2} \leq \bar{c}^p_\mc{M}\Delta x^2\left(\frac{1}{\Delta t}\frac{1}{\ubar{c}^p_\mc{A}\Delta x^2}+\frac{\mu}{\ubar{c}^p_\mc{M}\Delta x^2}\right)
  = \frac{1}{\Delta t}\frac{\bar{c}^p_\mc{M}}{\ubar{c}^p_\mc{A}} + \frac{\mu \bar{c}^p_\mc{M}}{\ubar{c}^p_\mc{M}}.
    % \left(\frac{1}{\Delta t}\frac{C^p_\mc{M}}{c^p_\mc{A}} + \frac{\mu}{\Delta x^2} \frac{C^p_\mc{A}}{c^p_\mc{A}}\right),
  \label{eqn::rightBoundP}
\end{equation}
The right bound on \cref{eqn::specBounds} is finally recovered by combining \cref{eqn::rightBoundP,eqn::rightBoundV}
\begin{equation}
  \frac{\left\langle\mc{B}\mc{F}_{\bb{u}}^{-1}\mc{B}^{T}\bb{q},\bb{q}\right\rangle}{\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\bb{q},\bb{q}\right\rangle}
  \leq \max\left\{\mu,1\right\}\left(\frac{1}{\mu\Delta t}\frac{\bar{c}^p_\mc{M}}{\ubar{c}^p_\mc{A}} + \frac{\bar{c}^p_\mc{M}}{\ubar{c}^p_\mc{M}}\right)
  = \bar{\sigma}^2.
    % \left(\frac{1}{\Delta t}\frac{C^p_\mc{M}}{c^p_\mc{A}} + \frac{\mu}{\Delta x^2} \frac{C^p_\mc{A}}{c^p_\mc{A}}\right),
  \label{eqn::rightBound}
\end{equation}


\paragraph{Lower bound}
To find an expression for the lower bound $\ubar{\sigma}^2$, we can make use of the discrete $\inf$-$\sup$ condition
\begin{equation}
  0<\gamma\leq\min_{\bb{q}\neq\bb{1}}\max_{\bb{v}\neq\bb{0}}\frac{|\left\langle\bb{q},\mc{B}\bb{v}\right\rangle|}{\|\bb{v}\|_{1}\|\bb{q}\|_0}, %= \min_{q_h\neq const }\max_{\bb{v}_h\neq 0} \frac{|\left\langle q_h, \mc{B}\bb{v}_h\right\rangle|}{\left\langle\mc{F}_{\bb{u}}\bb{v},\bb{v}\right\rangle^{\frac{1}{2}}\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}q,q\right\rangle^{\frac{1}{2}}} = 
  \label{eqn::infSup}
\end{equation}
where $\bb{1}$ denotes a vector filled with $1$ (representing a FE function constant over the whole domain). Starting from \cref{eqn::simplerRayleighQuotient} and using \cref{eqn::infSup} we obtain
\begin{equation}
  \frac{\left\langle\mc{B}\mc{F}_{\bb{u}}^{-1}\mc{B}^{T}\bb{q},\bb{q}\right\rangle^{\frac{1}{2}}}{\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\bb{q},\bb{q}\right\rangle^{\frac{1}{2}}}
  \opif{=}{(\bb{v}=\mc{F}_{\bb{u}}^{-1}\mc{B}^T\bb{q})}\frac{|\left\langle\bb{q},\mc{B}\bb{v}\right\rangle|}{\|\bb{q}\|_p\|\bb{v}\|_\bb{u}}
  \geq \min_{\bb{q}\neq\bb{1}}\max_{\bb{v}\neq\bb{0}}\frac{|\left\langle\bb{q},\mc{B}\bb{v}\right\rangle|}{\|\bb{q}\|_p\|\bb{v}\|_\bb{u}}
  \geq \gamma\frac{\|\bb{q}\|_0}{\|\bb{q}\|_p}\frac{\|\bb{v}\|_1}{\|\bb{v}\|_\bb{u}},
  \label{eqn::leftBoundTemp}
\end{equation}
which once again leaves us with the task of proving equivalence of norms.
For the velocity norms, we can exploit Poincar\'e's inequality:
\begin{equation}
\begin{split}
  \|\bb{v}\|_1^2
  & \geq \frac{1}{2c_p^2}\|\bb{v}\|_0^2 + \frac{1}{2}\|\bb{v}\|_1^2
  = \frac{\Delta t}{2c_p^2}\frac{\left\langle\mc{M}_{\bb{u}}\bb{v},\bb{v}\right\rangle}{\Delta t} + \frac{1}{2\mu}\mu\left\langle\mc{A}_{\bb{u}}\bb{v},\bb{v}\right\rangle\\
  & \geq \frac{1}{2}\min\left\{\frac{\Delta t}{c_p^2},\frac{1}{\mu}\right\} \|\bb{v}\|_{\bb{u}}^2,
\end{split}
  \label{eqn::leftBoundV}
\end{equation}
where $c_p$ is Poincar\'e's constant, such that $\|\bb{v}\|_0 \leq c_p \|\bb{v}\|_1$.
For the pressure norms we can follow a similar derivation as for the upper bound \cref{eqn::rightBoundP}, and recover
\begin{equation}
  \frac{\|\bb{q}\|_0^2}{\|\bb{q}\|_p^2} \geq \ubar{c}^p_\mc{M}\Delta x^2\left(\frac{1}{\bar{c}^p_\mc{A}\Delta t} + \frac{\mu}{\bar{c}^p_\mc{M}\Delta x^2}\right)
  = \frac{\Delta x^2}{\Delta t}\frac{\ubar{c}^p_\mc{M}}{\bar{c}^p_\mc{A}} + \mu\frac{\ubar{c}^p_\mc{M}}{\bar{c}^p_\mc{M}}.
  % \frac{\|q\|_0^2}{\|q\|_p^2}
  % \geq \frac{1}{\Delta t}\frac{\lambda^{min}(\mc{M}_p)}{\lambda^{max}(\mc{A}_p)} + \mu \frac{\lambda^{min}(\mc{A}_p)}{\lambda^{max}(\mc{A}_p)}
  % \geq \frac{\Delta x^2}{\Delta t}\frac{c^p_\mc{M}}{C^p_\mc{A}} + \mu\Delta x^2 \frac{c^p_\mc{A}}{C^p_\mc{A}}
  \label{eqn::leftBoundP}
\end{equation}
Combining the two bounds \cref{eqn::leftBoundV,eqn::leftBoundP}, and substituting them in \cref{eqn::leftBoundTemp} provides a lower bound for \cref{eqn::specBounds}:
\begin{equation}
  \frac{\left\langle\mc{B}\mc{F}_{\bb{u}}^{-1}\mc{B}^{T}\bb{q},\bb{q}\right\rangle}{\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\bb{q},\bb{q}\right\rangle}
  \geq \frac{\gamma^2}{2}\min\left\{1,\frac{\mu\Delta t}{c_p^2}\right\}\left(\frac{\Delta x^2}{\mu\Delta t}\frac{\ubar{c}^p_\mc{M}}{\bar{c}^p_\mc{A}}+\frac{\ubar{c}^p_\mc{M}}{\bar{c}^p_\mc{M}}\right) = \ubar{\sigma}^2.
  \label{eqn::leftBound}
\end{equation}

Collecting the results from \cref{eqn::rightBound,eqn::leftBound}, and assuming $\mu$ and $\Delta t$ small enough, we get
\begin{equation}
\frac{\gamma^2}{2c_p^2}\left(\Delta x^2\frac{\ubar{c}^p_\mc{M}}{\bar{c}^p_\mc{A}}+\mu\Delta t\frac{\ubar{c}^p_\mc{M}}{\bar{c}^p_\mc{M}}\right)
  \leq \frac{\left\langle\mc{B}\mc{F}_{\bb{u}}^{-1}\mc{B}^{T}\bb{q},\bb{q}\right\rangle}{\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\bb{q},\bb{q}\right\rangle}
  \leq \frac{1}{\mu\Delta t}\frac{\bar{c}^p_\mc{M}}{\ubar{c}^p_\mc{A}} + \frac{\bar{c}^p_\mc{M}}{\ubar{c}^p_\mc{M}}.
  \label{eqn::leftRightBound}
\end{equation}
For certain regimes, this proves the spectral equivalence of the matrices in \cref{eqn::blockGEP}, which in turn bounds the eigenvalues of \cref{eqn::blockGEP} and gives an indication of the effectiveness of the whole space-time preconditioners \cref{eqn::PT} or \cref{eqn::PD}. However, the quality of both bounds degrades with $\Delta t\to 0$. In light of this, it is reasonable to expect some degradation in the acceleration properties when refining the time discretisation.


\tcr{
\begin{itemize}
  \item Comment on the usefulness of the bound? It seems weird to me: the operators I'm analysing are exactly the same as those that would appear in the single time-step case (pressure reaction-diffusion, where the "reaction" bit comes from the time-derivative discretisation), so what does this mean? Did people observe degradation of performance also in that case? Or are the bounds I'm recovering very much not tight?
\end{itemize}
}

\begin{figure}
\centering
\begin{tikzpicture}[baseline, scale=0.7]
    \begin{semilogxaxis}[tick label style={font=\small},
        xlabel= $\Re(\lambda)$,
        ylabel= $\Im(\lambda)$,
        axis background/.style={fill=gray!10},
        cycle list = { {black,mark=o}, { blue, mark=o}, { red, mark=o}, { green, mark=o}},
        xmin = 0.3, xmax = 1.7, ymin = -1, ymax = 1,
        xmajorgrids= true,
        legend = north west,
        each nth point=100, filter discard warning=false,
        legend style={font=\small} ]   
        % cycle list = {{YlGnBu-E,mark=o},{YlGnBu-G,mark=o},{YlGnBu-I,mark=o},{YlGnBu-L,mark=o}},
        \addplot table[scatter,only marks, x index=1, y index=0]{data/Pb2_Prec1_STsolve0_oU2_oP1/eigs_r6.dat};
        \addplot table[scatter,only marks, x index=3, y index=2]{data/Pb2_Prec1_STsolve0_oU2_oP1/eigs_r6.dat};
        \addplot table[scatter,only marks, x index=5, y index=4]{data/Pb2_Prec1_STsolve0_oU2_oP1/eigs_r6.dat};
        \addplot table[scatter,only marks, x index=7, y index=6]{data/Pb2_Prec1_STsolve0_oU2_oP1/eigs_r6.dat};
        \addlegendentry{$\Delta t=10^{-3}$}
        \addlegendentry{$\Delta t=10^{-2}$}
        \addlegendentry{$\Delta t=10^{-1}$}
        \addlegendentry{$\Delta t=10^{ 0}$}
    \end{semilogxaxis}
\end{tikzpicture}
\caption{\label{fig::} Eigenvalue distribution of operator \cref{eqn::blockGEP} for varying values of $\Delta t$. Eigenvalues computed numerically using MATLAB function \texttt{eigs}. The operator refers to Pb.~2 in \cref{sec::modelProblems}, for a space discretisation with $\Delta x=2^{-6}$. Most of the eigenvalues are barely distinguishable, as they overlap almost exactly even by varying $\Delta t$.}
\end{figure}




% If we now introduce a \emph{modified} discrete $\inf$-$\sup$ condition, namely
% \begin{equation}
%   0<\tilde{\gamma}\leq\min_{\bb{q}\neq\bb{1}}\max_{\bb{v}\neq\bb{0}}\frac{|\left\langle\bb{q},\mc{B}\bb{v}\right\rangle|}{\|\bb{v}\|_{\bb{u}}\|\bb{q}\|_p}, %= \min_{q_h\neq const }\max_{\bb{v}_h\neq 0} \frac{|\left\langle q_h, \mc{B}\bb{v}_h\right\rangle|}{\left\langle\mc{F}_{\bb{u}}\bb{v},\bb{v}\right\rangle^{\frac{1}{2}}\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}q,q\right\rangle^{\frac{1}{2}}} = 
%   \label{eqn::modInfSup}
% \end{equation}
% where $\bb{1}$ denotes a vector filled with $1$ (representing a FE function constant over the whole domain), then we can follow the definitions of the norms \cref{eqn::norms} and recover
% \begin{equation}
% \begin{split}
%   \tilde{\gamma}&\leq\min_{\bb{q}\neq\bb{1}}\max_{\bb{v}\neq\bb{0}}\frac{|\left\langle\bb{q},\mc{B}\bb{v}\right\rangle|}{\left\langle\mc{F}_{\bb{u}}\bb{v},\bb{v}\right\rangle^{\frac{1}{2}}\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\bb{q},\bb{q}\right\rangle^{\frac{1}{2}}}\\
%                 &=\min_{\bb{q}\neq\bb{1}}\frac{1}{\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\bb{q},\bb{q}\right\rangle^{\frac{1}{2}}}\max_{\bb{w}=\mc{F}_{\bb{u}}^{\frac{1}{2}}\bb{v}\neq\bb{0}}\frac{\left|\left\langle\mc{F}_{\bb{u}}^{-\frac{1}{2}}\mc{B}^T\bb{q},\bb{w}\right\rangle\right|}{\left\langle\bb{w},\bb{w}\right\rangle^{\frac{1}{2}}}\\
%                 &=\min_{\bb{q}\neq\bb{1}}\frac{\left\langle\mc{B}\mc{F}_{\bb{u}}^{-1}\mc{B}^T\bb{q},\bb{q}\right\rangle^{\frac{1}{2}}}{\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\bb{q},\bb{q}\right\rangle^{\frac{1}{2}}},
%          % & = \min_{q\neq const} \frac{\left\langle\mc{M}_{p}^{-1}\mc{F}_{p}\mc{A}_{p}^{-1}\mc{B}\mc{F}_{\bb{u}}^{-1}\mc{B}^Tq,q\right\rangle^{\frac{1}{2}}}{\left\langle q,q\right\rangle^{\frac{1}{2}}}\\
%   \label{eqn::leftBound1}
% \end{split}
% \end{equation}
% so that the left bound in \cref{eqn::specBounds} is guaranteed, by imposing $\ubar{\sigma}^2=\tilde{\gamma}^2$. Regarding the right bound, we can use Cauchy-Schwarz on the numerator in \cref{eqn::modInfSup} to recover
% \begin{equation}
%   |\left\langle\bb{q},\mc{B}\bb{v}\right\rangle| \leq \|\bb{q}\|_0 \|\mc{B}\bb{v}\|_0 = \|\bb{q}\|_0 \|\nabla\cdot\bb{v}\|_0,
%   \label{eqn::rightBound0}
% \end{equation}
% where $\|*\|_0$ represents the Euclidean norm
% at which point recovering the bound becomes an exercise in proving equivalence of norms. In particular, for the velocity, we have
% \begin{equation}
%   \|\nabla\cdot\bb{v}\|_0^2 \leq \|\nabla\cdot\bb{v}\|_0^2 + \|\nabla\times\bb{v}\|_0^2 = \|\nabla\bb{v}\|^2_0\leq\mu^{-1}\|\bb{v}\|_{\bb{u}}^2,
%   % \label{eqn::rightBoundV}
% \end{equation}
% where $\|\bb{v}\|_1^2 = \|\bb{v}\|_0^2 + \|\nabla\bb{v}\|_0^2$ is the $H^1$-norm. For the pressure variable, we have instead
% \begin{equation}
%   \frac{\|\bb{q}\|_0^2}{\|\bb{q}\|_p^2}
%   =   \frac{\left\langle\mc{M}_{p}q,q\right\rangle}{\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}q,q\right\rangle}
%   \leq\frac{\max_{\bb{q}\in Q_h(\Omega)}|W(\mc{M}_{p})|}{\min_{\bb{q}\in Q_h(\Omega)}|W\left(\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\right)|},
%   % = \frac{\left\langle\mc{M}_{p}q,q\right\rangle}{\left\langle\mc{\tilde{F}}_{p}^{-1}q,q\right\rangle}
%   % = \frac{W(\mc{M}_{p})}{W\left(\left(\frac{\mc{A}_{p}^{-1}}{\Delta t}+\mu\mc{M}_{p}^{-1}\right)^{-1}\right)},
%   % = \frac{\left\langle\left(\mc{M}_{p}+\tau\mc{A}_{p}\right)q,q\right\rangle}{\left\langle\mc{A}_{p}q,q\right\rangle}
%   %   = \left(\frac{\left\langle\mc{M}_{p}q,q\right\rangle}{\Delta t\left\langle q,q\right\rangle}+\mu\frac{\left\langle\mc{A}_{p}q,q\right\rangle}{\left\langle q,q\right\rangle}\right)\left(\frac{\left\langle\mc{A}_{p}q,q\right\rangle}{\left\langle q,q\right\rangle}\right)^{-1}\\
%   % & \leq \frac{1}{\Delta t}\frac{\lambda^{max}(\mc{M}_p)}{\lambda^{min}(\mc{A}_p)} + \mu \frac{\lambda^{max}(\mc{A}_p)}{\lambda^{min}(\mc{A}_p)}
%   % \leq \frac{C^p_\mc{M}}{c^p_\mc{A}} + \tau \\
%   % \Longrightarrow & \|q\|_0^2 \leq  \left(\frac{C^p_\mc{M}}{c^p_\mc{A}} + \tau \right)\|q\|_p^2,
%   \label{eqn::rightBoundPtemp}
% \end{equation}
% with $W(*)$ denoting the \emph{field of values} of matrix $(*)$. The operators involved are symmetric, so their field of values is trivial, and coincides with the interval on the real line containing their eigenvalues:
% \begin{equation}
% \begin{split}
%    W\left(\mc{M}_p\right)&\subseteq\left[\ubar\lambda\left(\mc{M        }_p     \right),\bar\lambda\left(\mc{M        }_p     \right)\right],\quad\quad\text{and}\\
%    W\left(\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\right)&\subseteq\left[\ubar\lambda\left(\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\right),\bar\lambda\left(\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}\right)\right] = \left(W\left(\mc{A}_{p}^{-1}\mc{F}_{p}\mc{M}_{p}^{-1}\right)\right)^{-1},
%   % & W\left(\mc{\tilde{F}}^{-1}_p\right)\subseteq\left[\ubar\lambda\left(\mc{\tilde{F}}_p^{-1}\right),\bar\lambda\left(\mc{\tilde{F}}_p^{-1}\right)\right]
%   %   = \left(W\left(\mc{\tilde{F}}_p\right)\right)^{-1}
%   %   % = \left[\bar\lambda\left(\mc{\tilde{F}}_p\right)^{-1},\ubar\lambda\left(\mc{\tilde{F}}_p\right)^{-1}\right],
%     % =\left[\lambda^{min}\left(\mc{\tilde{F}}_p^{-1}\right),\lambda^{max}\left(\mc{\tilde{F}}_p^{-1}\right)\right]
% \end{split}
% \label{eqn::FOVp}
% \end{equation}
% where $\ubar\lambda(*)$ and $\bar\lambda(*)$ represent respectively the minimum and maximum eigenvalue of matrix $(*)$, while
% \begin{equation}
%   (W(*))^{-1}=\{r^{-1}:r\in W(*)\}.
% \end{equation}
% Using sub-additivity of the field of values, we have then
% \begin{equation}
% \begin{split}
%   W\left(\mc{A}_{p}^{-1}\mc{F}_{p}\mc{M}_{p}^{-1}\right)&= W\left(\frac{\mc{A}_{p}^{-1}}{\Delta t}+\mu\mc{M}_{p}^{-1}\right)\subseteq \frac{1}{\Delta t}W(\mc{A}_p^{-1}) + \mu W(\mc{M}_p^{-1})\\
%   &\subseteq\left[\frac{\Delta t^{-1}}{\bar\lambda(\mc{A}_p)} + \frac{\mu}{\bar\lambda(\mc{M}_p)}, \frac{\Delta t^{-1}}{\ubar\lambda(\mc{A}_p)} + \frac{\mu}{\ubar\lambda(\mc{M}_p)}\right].
% \end{split}
% \label{eqn::FOVp2}
% \end{equation}
% The last ingredient we need, is a bound on the eigenvalues of the Galerkin mass and stiffness matrices: these are given by
% \begin{equation}
% \begin{array}{lcccll}
%   c_\mc{M}^{(*)} \Delta x^2 & \leq & \lambda(\mc{M}_{(*)}) & \leq & C_\mc{M}^{(*)} \Delta x^2 &\quad\quad\text{\cite[Prop.1.30]{andyFIT}}\\
%   c_\mc{A}^{(*)} \Delta x^2 & \leq & \lambda(\mc{A}_{(*)}) & \leq & C_\mc{A}^{(*)}            &\quad\quad\text{\cite[Thm.1.33]{andyFIT} },
%   % c_\mc{B}       h^2 & \leq & \lambda(\mc{B}\mc{B}^T) & \leq & C_\mc{B}           &\quad\quad\textcolor{red}{\text{Well, this must be proven...}}\\
%   \label{eqn::massStiffBound}
% \end{array}
% \end{equation}
% they hold both for pressure and velocity, $(*)=p$ or $(*)=\bb{u}$, and are valid for a \textcolor{red}{quasi-uniform} discretisation defined on a regular 2D domain, with mesh size $\Delta x$ \tcr{but what if Ap is assembled weirdly? Do similar bounds still hold?}.
% Combining \cref{eqn::massStiffBound} for the pressure variable with \cref{eqn::FOVp} and \cref{eqn::FOVp2}, and substituting everything in \cref{eqn::rightBoundPtemp} gives the right bound
% \begin{equation}
%   \frac{\|q\|_0^2}{\|q\|_p^2} \leq C^p_\mc{M}\Delta x^2\left(\frac{1}{\Delta t}\frac{1}{c^p_\mc{A}\Delta x^2} + \frac{\mu}{c^p_\mc{M}\Delta x^2}\right)
%   = \frac{1}{\Delta t}\frac{C^p_\mc{M}}{c^p_\mc{A}} + \frac{\mu C^p_\mc{M}}{c^p_\mc{M}}
%     % \left(\frac{1}{\Delta t}\frac{C^p_\mc{M}}{c^p_\mc{A}} + \frac{\mu}{\Delta x^2} \frac{C^p_\mc{A}}{c^p_\mc{A}}\right),
%   \label{eqn::rightBoundP}
% \end{equation}
% Backtracking the steps made in \cref{eqn::leftBound1} and using Cauchy-Schwarz we get
% \begin{equation}
%   \frac{\left\langle\mc{B}\mc{F}_{\bb{u}}^{-1}\mc{B}^{T}q,q\right\rangle^{\frac{1}{2}}}{\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}q,q\right\rangle^{\frac{1}{2}}}
%   \leq \frac{1}{\|q\|_p}\max_{\bb{w}\neq 0} \frac{|\left\langle q,\mc{B}\bb{w}\right\rangle|}{\|\bb{w}\|_{\bb{u}}}
%   \leq \max_{\bb{w}\neq 0} \frac{\|q\|_0\|\nabla\bb{w}\|_0}{\|\bb{w}\|_{\bb{u}}\|q\|_p};
% \end{equation}
% if we substitute the norm bounds \cref{eqn::rightBoundP} and \cref{eqn::rightBoundV}, we finally recover the right bound
% \begin{equation}
%   \frac{\left\langle\mc{B}\mc{F}_{\bb{u}}^{-1}\mc{B}^{T}q,q\right\rangle}{\left\langle\mc{A}_{p}\mc{F}_{p}^{-1}\mc{M}_{p}q,q\right\rangle}
%   \leq \frac{1}{\mu}\left(\frac{1}{\Delta t}\frac{C^p_\mc{M}}{c^p_\mc{A}} + \mu\frac{C^p_\mc{M}}{c^p_\mc{M}}\right) = \mu_1.
%   % \leq \max\left\{\frac{1}{\mu\Delta t}\frac{C^p_\mc{M}}{c^p_\mc{A}} + \frac{1}{\Delta x^2}           \frac{C^p_\mc{A}}{c^p_\mc{A}},\quad
%   %                                      \frac{C^p_\mc{M}}{c^p_\mc{A}} + \frac{\mu\Delta t}{\Delta x^2} \frac{C^p_\mc{A}}{c^p_\mc{A}}\right\} = \mu_1.
%   \label{eqn::rightBound}
% \end{equation}
% \textcolor{red}{The preconditioner is then dependent on $\tau=\mu\Delta t$, which kinda sucks: if $\Delta t\to 0$ we're doomed, unless the viscosity is huge.}

% If we further prove a bound on the equivalence of the norms \cref{eqn::norms} and \cref{eqn::rightBound0} also in the other direction, we can then bring back our \emph{modified} $\inf$-$\sup$ condition \cref{eqn::modInfSup} to the classical one. For the velocity norm we can exploit Poincar\'e's inequality:
% \begin{equation}
% \begin{split}
%   \|\nabla \bb{v}\|_0^2
%   & \geq \frac{1}{2c_p^2}\|\bb{v}\|_0^2 + \frac{1}{2}\|\nabla \bb{v}\|_0^2
%   = \frac{\Delta t}{2c_p^2}\frac{\left\langle\mc{M}_{\bb{u}}\bb{v},\bb{v}\right\rangle}{\Delta t} + \frac{1}{2\mu}\mu\left\langle\mc{A}_{\bb{u}}\bb{v},\bb{v}\right\rangle\\
%   & \geq \frac{1}{2}\min\left\{\frac{\Delta t}{c_p^2},\frac{1}{\mu}\right\} \|\bb{v}\|_{\bb{u}}^2,
% \end{split}
%   \label{eqn::leftBoundV}
% \end{equation}
% where $c_p$ is Poincar\'e's constant, such that $\|\bb{v}\|_0 \leq c_p \|\nabla\bb{v}\|_0$.
% For the pressure we can follow a similar derivation as for the upper bound \cref{eqn::rightBoundP}, and recover
% \begin{equation}
%   \frac{\|q\|_0^2}{\|q\|_p^2} \geq c^p_\mc{M}\Delta x^2\left(\frac{1}{\Delta t}\frac{1}{C^p_\mc{A}} + \frac{\mu}{C^p_\mc{M}\Delta x^2}\right)
%   = \frac{\Delta x^2}{\Delta t}\frac{c^p_\mc{M}}{C^p_\mc{A}} + \frac{\mu c^p_\mc{M}}{C^p_\mc{M}}
%   % \frac{\|q\|_0^2}{\|q\|_p^2}
%   % \geq \frac{1}{\Delta t}\frac{\lambda^{min}(\mc{M}_p)}{\lambda^{max}(\mc{A}_p)} + \mu \frac{\lambda^{min}(\mc{A}_p)}{\lambda^{max}(\mc{A}_p)}
%   % \geq \frac{\Delta x^2}{\Delta t}\frac{c^p_\mc{M}}{C^p_\mc{A}} + \mu\Delta x^2 \frac{c^p_\mc{A}}{C^p_\mc{A}}
%   \label{eqn::leftBoundP}
% \end{equation}
% Combining the two bounds and substituting them in \cref{eqn::modInfSup} provides
% \begin{equation}
% \begin{split}
%        & \min_{q_h\neq const }\max_{\bb{v}_h\neq 0} \frac{|\left\langle q_h, \nabla\cdot\bb{v}_h\right\rangle|^2}{\|\bb{v}_h\|_{\bb{u}}^2\|q_h\|_p^2}\\
%   \geq & \frac{1}{2}\min\left\{\frac{\Delta t}{c_p^2}, \frac{1}{\mu}\right\}\left(\frac{\Delta x^2}{\Delta t}\frac{c^p_\mc{M}}{C^p_\mc{A}} + \mu\frac{c^p_\mc{M}}{C^p_\mc{M}}\right) \min_{q_h\neq const }\max_{\bb{v}_h\neq 0} \frac{|\left\langle q_h, \nabla\cdot\bb{v}_h\right\rangle|^2}{\|\nabla\bb{v}_h\|_{0}^2\|q_h\|_0^2},
% \end{split}
% \end{equation}
% If we then impose the \emph{classical} $\inf$-$\sup$ condition, that is,
% $$\min_{q_h\neq const }\max_{\bb{v}_h\neq 0} \frac{|\left\langle q_h, \nabla\cdot\bb{v}_h\right\rangle|}{\|\nabla\bb{v}_h\|_{0}\|q_h\|_0}\geq \hat{\gamma}>0,$$
% we see that the lower bound in \cref{eqn::specBounds} is satisfied with
% \begin{equation}
%   \mu_0 = \frac{\hat{\gamma}^2}{2}\min\left\{\frac{\mu\Delta t}{c_p^2}, 1\right\}\left(\frac{\Delta x^2}{\mu\Delta t}\frac{c^p_\mc{M}}{C^p_\mc{A}} + \frac{c^p_\mc{M}}{C^p_\mc{M}}\right).
%   \label{eqn::leftBound}
% \end{equation}







\end{section}
